Non-Coherent Detection for Diffusive Molecular Communications

We study non-coherent detection schemes for molecular communication (MC) systems that do not require knowledge of the channel state information (CSI). In particular, we first derive the optimal maximum likelihood (ML) multiple-symbol (MS) detector for MC systems. As a special case of the optimal MS detector, we show that the optimal ML symbol-by-symbol (SS) detector can be equivalently written in the form of a threshold-based detector, where the optimal decision threshold is constant and depends only on the statistics of the MC channel. The main challenge of the MS detector is the complexity associated with the calculation of the optimal detection metric. To overcome this issue, we propose an approximate MS detection metric which can be expressed in closed form. To reduce complexity even further, we develop a non-coherent decision-feedback (DF) detector and a suboptimal blind detector. Finally, we derive analytical expressions for the bit error rate (BER) of the optimal SS detector, as well as upper and lower bounds for the BER of the optimal MS detector. Simulation results confirm the analysis and reveal the effectiveness of the proposed optimal and suboptimal detection schemes compared to a benchmark scheme that assumes perfect CSI knowledge, particularly when the number of observations used for detection is sufficiently large.

==> Fig/BER_K/BER_K.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA NC-BL}%
\psfrag{017}[cl][cl]{\matlabtextA NC-DF-AM}%
\psfrag{018}[cl][cl]{\matlabtextA NC-MS-AM}%
\psfrag{019}[cl][cl]{\matlabtextA NC-SS}%
\psfrag{020}[cl][cl]{\matlabtextA C-ML}%
\psfrag{021}[cl][cl]{\matlabtextA $\mathtt{SNR}=20$ dB}%
\psfrag{022}[cl][cl]{\matlabtextA $\mathtt{SNR}=10$ dB}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB Bit Error Rate}%
\psfrag{024}[tc][tc]{\matlabtextB $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $2$}%
\psfrag{001}[ct][ct]{\matlabtextC $4$}%
\psfrag{002}[ct][ct]{\matlabtextC $6$}%
\psfrag{003}[ct][ct]{\matlabtextC $8$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $12$}%
\psfrag{006}[ct][ct]{\matlabtextC $14$}%
\psfrag{007}[ct][ct]{\matlabtextC $16$}%
\psfrag{008}[ct][ct]{\matlabtextC $18$}%
\psfrag{009}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-5}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{012}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{013}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{014}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{015}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>

==> Fig/BER_Kappa/BER_Kappa.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA NC-DF-AM, Det. Window Size $K$}%
\psfrag{015}[cl][cl]{\matlabtextA NC-MS-AM, Det. Window Size $B$}%
\psfrag{016}[cl][cl]{\matlabtextA NC-MS-AM, Det. Window Size $K$}%
\psfrag{017}[cl][cl]{\matlabtextA C-ML}%
\psfrag{018}[cl][cl]{\matlabtextA Scenario 1}%
\psfrag{019}[cl][cl]{\matlabtextA Scenario 2}%
\psfrag{020}[cl][cl]{\matlabtextA Scenario 3}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Bit Error Rate}%
\psfrag{022}[tc][tc]{\matlabtextB $\kappa$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $1$}%
\psfrag{001}[ct][ct]{\matlabtextC $2$}%
\psfrag{002}[ct][ct]{\matlabtextC $3$}%
\psfrag{003}[ct][ct]{\matlabtextC $4$}%
\psfrag{004}[ct][ct]{\matlabtextC $5$}%
\psfrag{005}[ct][ct]{\matlabtextC $6$}%
\psfrag{006}[ct][ct]{\matlabtextC $7$}%
\psfrag{007}[ct][ct]{\matlabtextC $8$}%
\psfrag{008}[ct][ct]{\matlabtextC $9$}%
\psfrag{009}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{012}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{013}[rc][rc]{\matlabtextC $10^{-1}$}%
%
%% </ytick>

==> Fig/BER_SNR/BER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA NC-BL}%
\psfrag{010}[cl][cl]{\matlabtextA NC-DF-AM}%
\psfrag{011}[cl][cl]{\matlabtextA NC-MS-AM}%
\psfrag{012}[cl][cl]{\matlabtextA NC-SS}%
\psfrag{013}[cl][cl]{\matlabtextA C-ML}%
\psfrag{014}[cl][cl]{\matlabtextA $K=10$}%
\psfrag{015}[cl][cl]{\matlabtextA $K=5$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB Bit Error Rate}%
\psfrag{017}[tc][tc]{\matlabtextB $\mathtt{SNR}$ in dB}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{006}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-1}$}%
%
%% </ytick>

==> Fig/BER_SNR_Bound/BER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA UB (MS Upper Bound)}%
\psfrag{020}[cl][cl]{\matlabtextA GA-DF (MS Lower Bound)}%
\psfrag{021}[cl][cl]{\matlabtextA NC-MS-AM (Simulation)}%
\psfrag{022}[cl][cl]{\matlabtextA NC-MS-OM (Simulation)}%
\psfrag{023}[cl][cl]{\matlabtextA NC-SS (Analytical)}%
\psfrag{024}[cl][cl]{\matlabtextA NC-SS (Simulation)}%
\psfrag{025}[cl][cl]{\matlabtextA C-ML (Analytical)}%
\psfrag{026}[cl][cl]{\matlabtextA C-ML (Simulation)}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB Bit Error Rate}%
\psfrag{028}[tc][tc]{\matlabtextB $\mathtt{SNR}$ in dB}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $7.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $8$}%
\psfrag{002}[ct][ct]{\matlabtextC $8.5$}%
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{005}[ct][ct]{\matlabtextD $0$}%
\psfrag{006}[ct][ct]{\matlabtextD $2$}%
\psfrag{007}[ct][ct]{\matlabtextD $4$}%
\psfrag{008}[ct][ct]{\matlabtextD $6$}%
\psfrag{009}[ct][ct]{\matlabtextD $8$}%
\psfrag{010}[ct][ct]{\matlabtextD $10$}%
\psfrag{011}[ct][ct]{\matlabtextD $12$}%
\psfrag{012}[ct][ct]{\matlabtextD $14$}%
\psfrag{013}[ct][ct]{\matlabtextD $16$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextE{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{003}[rc][rc]{\matlabtextE $10^{0.0003}$}%
\psfrag{004}[rc][rc]{\matlabtextE $10^{0.003}$}%
%
\providecommand\matlabtextF{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[rc][rc]{\matlabtextF $10^{-4}$}%
\psfrag{015}[rc][rc]{\matlabtextF $10^{-3}$}%
\psfrag{016}[rc][rc]{\matlabtextF $10^{-2}$}%
\psfrag{017}[rc][rc]{\matlabtextF $10^{-1}$}%
\psfrag{018}[rc][rc]{\matlabtextF $10^{0}$}%
%
%% </ytick>

==> Fig/BER_SNR_ISI/BER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA NC-BL}%
\psfrag{017}[cl][cl]{\matlabtextA NC-MS-AM}%
\psfrag{018}[cl][cl]{\matlabtextA C-ML}%
\psfrag{019}[cl][cl]{\matlabtextA No ISI}%
\psfrag{020}[cl][cl]{\matlabtextA $T_{\mathtt{symb}}=10*T_{\mathtt{max}}$}%
\psfrag{021}[cl][cl]{\matlabtextA $T_{\mathtt{symb}}=5*T_{\mathtt{max}}$}%
\psfrag{022}[cl][cl]{\matlabtextA $T_{\mathtt{symb}}=2*T_{\mathtt{max}}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB Bit Error Rate}%
\psfrag{024}[tc][tc]{\matlabtextB $\mathtt{SNR}^{\mathtt{ext}}$ in dB}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $2$}%
\psfrag{002}[ct][ct]{\matlabtextC $4$}%
\psfrag{003}[ct][ct]{\matlabtextC $6$}%
\psfrag{004}[ct][ct]{\matlabtextC $8$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $12$}%
\psfrag{007}[ct][ct]{\matlabtextC $14$}%
\psfrag{008}[ct][ct]{\matlabtextC $16$}%
\psfrag{009}[ct][ct]{\matlabtextC $18$}%
\psfrag{010}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{012}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{013}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{014}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{015}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>

==> Fig/GammaPDF/GammaPDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA Deterministic Channel\hspace{0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA Levy Distribution\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA Inverse Gaussian Distribution\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Nakagami Distribution\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA Gamma Distribution\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Exact Distribution\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextB Scenario 3, $(\alpha^*,\beta^*)=(2.24,0.39)$}%
\psfrag{020}[cl][cl]{\matlabtextB Scenario 2, $(\alpha^*,\beta^*)=(3.87,0.83)$}%
\psfrag{021}[cl][cl]{\matlabtextB Scenario 1, $(\alpha^*,\beta^*)=(16.84,3.44)$}%
\psfrag{022}[bc][bc]{\matlabtextB Probability Density Function $f_x(x)$}%
\psfrag{023}[tc][tc]{\matlabtextB $x$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.15$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.25$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.35$}%
%
%% </ytick>

==> Fig/MSE/MSE.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA Gaussian Distribution}%
\psfrag{019}[cl][cl]{\matlabtextA Poisson Distribution}%
\psfrag{020}[cl][cl]{\matlabtextA Binomial Distribution}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Error}%
\psfrag{022}[tc][tc]{\matlabtextB $d$ (nm)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $249.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $250$}%
\psfrag{002}[ct][ct]{\matlabtextC $250.5$}%
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{005}[ct][ct]{\matlabtextD $100$}%
\psfrag{006}[ct][ct]{\matlabtextD $150$}%
\psfrag{007}[ct][ct]{\matlabtextD $200$}%
\psfrag{008}[ct][ct]{\matlabtextD $250$}%
\psfrag{009}[ct][ct]{\matlabtextD $300$}%
\psfrag{010}[ct][ct]{\matlabtextD $350$}%
\psfrag{011}[ct][ct]{\matlabtextD $400$}%
\psfrag{012}[ct][ct]{\matlabtextD $450$}%
\psfrag{013}[ct][ct]{\matlabtextD $500$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextE{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{003}[rc][rc]{\matlabtextE $10^{-1.853}$}%
\psfrag{004}[rc][rc]{\matlabtextE $10^{-1.845}$}%
%
\providecommand\matlabtextF{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[rc][rc]{\matlabtextF $10^{-3}$}%
\psfrag{015}[rc][rc]{\matlabtextF $10^{-2}$}%
\psfrag{016}[rc][rc]{\matlabtextF $10^{-1}$}%
\psfrag{017}[rc][rc]{\matlabtextF $10^{0}$}%
%
%% </ytick>

==> Fig/PDF/PDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{026}[cl][cl]{\matlabtextA Gaussian Distribution\hspace{0.5em}}%
\psfrag{027}[cl][cl]{\matlabtextA Poisson Distribution\hspace{0.5em}}%
\psfrag{028}[cl][cl]{\matlabtextA Binomial Distribution\hspace{0.5em}}%
\psfrag{029}[cl][cl]{\matlabtextA Particle-Based Simulation (Exact PDF)\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{030}[cl][cl]{\matlabtextB $d=300$ nm}%
\psfrag{031}[cl][cl]{\matlabtextB $d=400$ nm}%
\psfrag{032}[cl][cl]{\matlabtextB $d=500$ nm}%
\psfrag{033}[bc][bc]{\matlabtextB Probability Density Function}%
\psfrag{034}[tc][tc]{\matlabtextB $c_{\mathtt{s}}[k]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $11.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $12$}%
\psfrag{002}[ct][ct]{\matlabtextC $12.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $5$}%
\psfrag{009}[ct][ct]{\matlabtextC $10$}%
\psfrag{010}[ct][ct]{\matlabtextC $15$}%
\psfrag{011}[ct][ct]{\matlabtextC $20$}%
\psfrag{012}[ct][ct]{\matlabtextC $25$}%
\psfrag{013}[ct][ct]{\matlabtextC $30$}%
\psfrag{014}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0.07$}%
\psfrag{004}[rc][rc]{\matlabtextC $0.075$}%
\psfrag{005}[rc][rc]{\matlabtextC $0.08$}%
\psfrag{015}[rc][rc]{\matlabtextC $0$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.04$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.06$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.08$}%
\psfrag{020}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{021}[rc][rc]{\matlabtextC $0.12$}%
\psfrag{022}[rc][rc]{\matlabtextC $0.14$}%
\psfrag{023}[rc][rc]{\matlabtextC $0.16$}%
\psfrag{024}[rc][rc]{\matlabtextC $0.18$}%
\psfrag{025}[rc][rc]{\matlabtextC $0.2$}%
%
%% </ytick>
